GPUPHOT: A Python Framework for High-Performance GPU-Accelerated Photometry and Distributed Astronomical Data Reduction

We present GPUPHOT, an open-source Python framework for GPU-accelerated real-time photometry and astrometry of astronomical CCD and scientific CMOS images. Four of its seven stages run entirely on the GPU through CuPy (background estimation, source detection, PSF modeling and aperture photometry); the catalog crossmatch selects a CPU or GPU backend by problem size, and the zero-point and astrometric calibrations run on the CPU, within a containerized distributed system. Checkpoint-based GPU memory monitoring and an opt-in spatial-binning fallback let a single container image run on GPUs from a 4 GB laptop card to 80 GB datacenter accelerators. We benchmark the framework on nineteen observations from two robotic facilities, the Two-meter Twin Telescope and the Transient Survey Telescope, spanning 4.2 to 151.2 megapixels and 228 to 134,206 cataloged sources, on eight NVIDIA GPU platforms with one process per image. The H100 completes the densest 151.2-megapixel field end-to-end in 31.9 s, and GPU source detection on the A100 is 6-15x faster than the CPU library sep on the same frames. Once three sources of non-determinism are pinned, catalogs and zero points agree to the fourth decimal across GPU models and host CPUs. In this one-process-per-image regime the CuPy 14 / cuML stack showed a 7% lower peak memory and a median 38% higher per-image latency than CuPy 12, both due to the RAPIDS allocator displacing the CuPy memory pool at import; restoring the pool removes the memory difference and cuts the median overhead on datacenter GPUs to 11%, with identical output. Long-lived workers, the production mode, run the two stacks near parity. We recommend the CuPy 14 stack for its reproducibility and maintained libraries, not for memory or speed. GPUPHOT and its benchmark scripts are released for autonomous facilities that require end-to-end photometric reduction at survey cadence.

==> tables_generated/body_concurrency.tex <==
\begin{tabular}{lrrrr}
\toprule
\textbf{GPU} & \textbf{VRAM (GB)} & \textbf{py3.8} & \textbf{py3.12} & \textbf{Gain (\%)} \\
\midrule
H100           & 80 & 41 & 49 & $+20$\,\% \\
A100           & 80 & 42 & 49 & $+17$\,\% \\
L40S           & 48 & 23 & 27 & $+17$\,\% \\
RTX 3090       & 24 & 12 & 14 & $+17$\,\% \\
RTX 3060       & 12 &  6 &  7 & $+17$\,\% \\
RTX 3050 Ti    &  4 &  1 &  2 & $+100$\,\% \\
\bottomrule
\end{tabular}

